Dense Reward for Multi-View 3D Reasoning with Global Maps and Local Views

Multi-view 3D Visual Question Answering (MV3D-VQA) requires integrating partial observations into a coherent 3D scene representation and selecting informative viewpoints for multi-step spatial reasoning. However, current multimodal LLMs are typically trained with sparse, answer-level supervision, which often yields inconsistent cross-view reasoning and brittle view selection. We present DR-MV3D (Dense Reward for MV3D-VQA), a map-grounded learning framework that provides dense, verifiable rewards to supervise the reasoning process. Our approach decomposes MV3D-VQA into (i) allocentric global map construction, (ii) question-conditioned view-trajectory planning, and (iii) egocentric grounding for answer prediction. To make intermediate steps learnable without manual annotations, we introduce two rewards: a global consistency reward that aligns the predicted map with geometry-consistent pseudo targets from frozen 3D vision foundation models (e.g., VGGT + SAM3), and a local trajectory reward that supervises ordered viewpoint selection. We optimize the full pipeline with trajectory-level policy optimization (GRPO). Experiments on MindCube, VSI-Bench, and BLINK (MV) show that DR-MV3D consistently improves over strong multi-image baselines, supporting the effectiveness of process-level dense supervision for multi-view 3D reasoning.

==> assets/cogmap/GT/among_group458_q1_5_1_cogmap_tikz.tex <==
% 10x10 cognitive map for among_group458_q1_5_1 (compact + decluttered style)
\begin{tikzpicture}[font=\fontsize{5.4}{6.0}\selectfont\sffamily]
  % [0,0] at top-left, y increases downward
  \begin{scope}[x=0.46cm,y=-0.46cm]
    % Grid lines
    \foreach \x in {0,...,10} {\draw[gray!40,line width=0.28pt] (\x,0) -- (\x,10);}
    \foreach \y in {0,...,10} {\draw[gray!40,line width=0.28pt] (0,\y) -- (10,\y);}
    \draw[black,line width=0.75pt] (0,0) rectangle (10,10);

    % Minimal axis ticks (every 2 cells)
    % \foreach \x in {0,2,4,6,8} {\node[anchor=north] at (\x,10.16) {\x};}
    % \foreach \y in {0,2,4,6,8} {\node[anchor=east] at (-0.16,\y) {\y};}

    % Colors for selected-view ego direction
    \definecolor{selView}{RGB}{226,140,28}
    % \definecolor{egoF}{RGB}{216,68,55}
    % \definecolor{egoB}{RGB}{64,110,185}
    % \definecolor{egoL}{RGB}{226,140,28}
    % \definecolor{egoR}{RGB}{44,158,78}

    % Styles
    \tikzset{
      objdot/.style={draw=black!60,line width=0.35pt,circle,minimum size=4.4pt,inner sep=0pt},
      objlabel/.style={draw=black!45,fill=white,rounded corners=1.0pt,inner sep=1.0pt,align=center},
      callout/.style={black!55,line width=0.34pt,dash pattern=on 1pt off 1pt},
      innerwhite/.style={fill=white, draw=black, line width=0.25pt},
    }

    % ----- Object points -----
    \definecolor{colBottle}{RGB}{255, 92, 135}
    \definecolor{colWindow}{RGB}{80, 150, 255}
    \definecolor{colWall}{RGB}{235, 225, 48}
    \definecolor{colPlush}{RGB}{241, 113, 75}
    \definecolor{colCloset}{RGB}{50, 180, 90}

    \node[objdot,fill=colBottle]         (objBottle) at (5,5) {};
    \node[objdot,fill=colWall] (objWall) at (5,2) {};
    \node[objdot,fill=colWindow]        (objWindow)   at (2,5) {};
    \node[objdot,fill=colPlush]        (objPlush) at (8,5) {};
    \node[objdot,fill=colCloset]      (objCloset)  at (5,8) {};



    % Label anchor coordinates
    %  \coordinate (labWallPos)   at (4.50,9.08);
    % \coordinate (labBottlePos) at (3.55,6.92);
    % \coordinate (labClosetPos) at (8.52,6.88);
    % \coordinate (labWindowPos) at (1.35,2.88);
    % \coordinate (labPlushPos)  at (5.50,1.00);

    \coordinate (labWallPos)   at (5.50,1.00);
    \coordinate (labBottlePos) at (3.55,6.92);
    \coordinate (labClosetPos) at (4.50,9.08);
    \coordinate (labWindowPos) at (1.35,2.88);
    \coordinate (labPlushPos)  at (8.52,6.88);

    % ----- Callout lines first (to be hidden under white label boxes) -----
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labWallPos) -- (objWall.center);
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labBottlePos) -- (objBottle.center);
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labClosetPos) -- (objCloset.center);
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labWindowPos) -- (objWindow.center);
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labPlushPos) -- (objPlush.center);

    % ----- Object labels -----
    \node[objlabel] at (labWallPos) {window and blue curtain\\(forward)};
    \node[objlabel] at (labBottlePos) {pink\\bottle\\{(forward)}};
    \node[objlabel] at (labClosetPos) {closet and door\\(back)};
    \node[objlabel] at (labWindowPos) {white wall\\(forward-left)};
    \node[objlabel] at (labPlushPos) {pink plush toy \\and headboard\\(forward-right)};

    % ----- Views: numbered white squares + arrows starting at box edge -----

    \def\boxSq{0.34} % half-size of the square
    \tikzset{
      viewone/.style={draw=black, fill=white, line width=0.45pt},
      viewselect/.style={draw=black, fill=selView!12, line width=0.45pt},
      viewnum/.style={font=\bfseries\fontsize{5.0}{5.0}\selectfont\sffamily}
    }
    
    % Image 2 at (5,7), arrow goes UP (toward smaller y)
    \path[viewone] (5-\boxSq,7-\boxSq) rectangle (5+\boxSq,7+\boxSq);
    \node[viewselect] at (5,7) {1};
    \node[fill=selView!12,text=selView!80!black,rounded corners=0.6pt,inner sep=0.25pt,anchor=west,align=center] at (5.50,7.00) {\textbf{selected}};
    \draw[-{Latex[length=2.25mm]},black!75,line width=0.95pt]
      (5,7-\boxSq) -- (5,5.75);
    
    % Image 3 at (3,5), arrow goes RIGHT (toward larger x)
    \path[viewone] (3-\boxSq,5-\boxSq) rectangle (3+\boxSq,5+\boxSq);
    \node[viewnum] at (3,5) {2};
    \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt]
      (3+\boxSq,5) -- (4.25,5);
    
    % Image 4 at (5,3), arrow goes DOWN (toward larger y)
    \path[viewone] (5-\boxSq,3-\boxSq) rectangle (5+\boxSq,3+\boxSq);
    \node[viewnum] at (5,3) {3};
    \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt]
      (5,3+\boxSq) -- (5,4.25);
    
    % Image 1 at (7,5), arrow goes LEFT (toward smaller x)
    \path[viewone] (7-\boxSq,5-\boxSq) rectangle (7+\boxSq,5+\boxSq);
    \node[viewnum] at (7,5) {4};
    \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt]
      (7-\boxSq,5) -- (5.75,5);
    
  
    % ----- Tiny ego-direction compass near selected view -----
    % Facing right: F=+x, B=-x, L=-y, R=+y in map coordinates
    \coordinate (egoC) at (9.00,9.00);
    \fill[selView] (egoC) circle (0.05);
    \draw[-{Latex[length=1.4mm]},line width=0.55pt] (egoC) -- ++(0.36,0);
    \draw[-{Latex[length=1.4mm]},line width=0.55pt] (egoC) -- ++(-0.36,0);
    \draw[-{Latex[length=1.4mm]},line width=0.55pt] (egoC) -- ++(0,-0.36);
    \draw[-{Latex[length=1.4mm]},line width=0.55pt] (egoC) -- ++(0,0.36);
    \node[anchor=west]  at ($(egoC)+(0.25,0)$) {R};
    \node[anchor=east]  at ($(egoC)+(-0.25,0)$) {L};
    \node[anchor=south] at ($(egoC)+(0,-0.2)$) {F};
    \node[anchor=north] at ($(egoC)+(0,0.2)$) {B};
  \end{scope}
\end{tikzpicture}

==> assets/cogmap/VFM/among_group458_q1_5_1_cogmap_tikz.tex <==
% 10x10 cognitive map for among_group458_q1_5_1 (compact + decluttered style)
\begin{tikzpicture}[font=\fontsize{5.4}{6.0}\selectfont\sffamily]
  % [0,0] at top-left, y increases downward
  \begin{scope}[x=0.46cm,y=-0.46cm]
    % Grid lines
    \foreach \x in {0,...,10} {\draw[gray!40,line width=0.28pt] (\x,0) -- (\x,10);}
    \foreach \y in {0,...,10} {\draw[gray!40,line width=0.28pt] (0,\y) -- (10,\y);}
    \draw[black,line width=0.75pt] (0,0) rectangle (10,10);

    % Minimal axis ticks (every 2 cells)
    % \foreach \x in {0,2,4,6,8} {\node[anchor=north] at (\x,10.16) {\x};}
    % \foreach \y in {0,2,4,6,8} {\node[anchor=east] at (-0.16,\y) {\y};}

    % Colors for selected-view ego direction
    \definecolor{selView}{RGB}{60, 154, 86}
    \definecolor{selWrong}{RGB}{210,76,58}
    % \definecolor{egoF}{RGB}{216,68,55}
    % \definecolor{egoB}{RGB}{64,110,185}
    % \definecolor{egoL}{RGB}{226,140,28}
    % \definecolor{egoR}{RGB}{44,158,78}

    % Styles
    \tikzset{
      objdot/.style={draw=black!60,line width=0.35pt,circle,minimum size=4.4pt,inner sep=0pt},
      objlabel/.style={draw=black!45,fill=white,rounded corners=1.0pt,inner sep=1.0pt,align=center},
      callout/.style={black!55,line width=0.34pt,dash pattern=on 1pt off 1pt},
      innerwhite/.style={fill=white, draw=black, line width=0.25pt},
    }

    % ----- Object points -----
    \definecolor{colBottle}{RGB}{255, 92, 135}
    \definecolor{colWindow}{RGB}{80, 150, 255}
    \definecolor{colWall}{RGB}{235, 225, 48}
    \definecolor{colPlush}{RGB}{241, 113, 75}
    \definecolor{colCloset}{RGB}{50, 180, 90}

    \node[objdot,fill=colBottle]         (objBottle) at (5,5) {};
    \node[objdot,fill=colWall] (objWall) at (5,2) {};
    \node[objdot,fill=colWindow]        (objWindow)   at (2,7) {};
    \node[objdot,fill=colPlush]        (objPlush) at (8,5) {};
    \node[objdot,fill=colCloset]      (objCloset)  at (5,8) {};


    % Label anchor coordinates
    % \coordinate (labWallPos)   at (1.05,4.20);
    % \coordinate (labBottlePos) at (3.55,6.92);
    % \coordinate (labClosetPos) at (5.00,9.08);
    % \coordinate (labWindowPos) at (5.00,1.00);
    % \coordinate (labPlushPos)  at (8.52,3.88);

     \coordinate (labWallPos)   at (5.50,1.00);
    \coordinate (labBottlePos) at (3.55,6.92);
    \coordinate (labClosetPos) at (4.50,9.08);
    \coordinate (labWindowPos) at (1.35,4.88);
    \coordinate (labPlushPos)  at (8.52,6.88);


    % ----- Callout lines first (to be hidden under white label boxes) -----
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labWallPos) -- (objWall.center);
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labBottlePos) -- (objBottle.center);
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labClosetPos) -- (objCloset.center);
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labWindowPos) -- (objWindow.center);
    \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labPlushPos) -- (objPlush.center);

    % ----- Object labels -----
    \node[objlabel] at (labWallPos) {\textcolor{selView}{window and} \textcolor{selView}{blue curtain}\\ \textcolor{selView}{(forward)}};
    \node[objlabel] at (labBottlePos) {\textcolor{selView}{pink}\\ \textcolor{selView}{bottle}\\ \textcolor{selView}{(forward)}};
    \node[objlabel] at (labClosetPos) { \textcolor{selView}{closet and door}\\ \textcolor{selView}{(back)}};
    \node[objlabel] at (labWindowPos) {\textcolor{selView}{white wall}\\ \textcolor{selWrong}{(left)}};
    \node[objlabel] at (labPlushPos) {\textcolor{selView}{pink plush toy}\\ \textcolor{selView}{and headboard}\\ \textcolor{selView}{(forward-right)}};

    % ----- Views: numbered white squares + arrows starting at box edge -----

    \def\boxSq{0.34} % half-size of the square
    \tikzset{
      viewone/.style={draw=black, fill=white, line width=0.45pt},
      viewselect/.style={draw=black, fill=selView!12, line width=0.45pt},
      viewnum/.style={font=\bfseries\fontsize{5.0}{5.0}\selectfont\sffamily}
    }
    
    % Image 2 at (5,7), arrow goes UP (toward smaller y)
    \path[viewone] (5-\boxSq,7-\boxSq) rectangle (5+\boxSq,7+\boxSq);
    \node[viewselect] at (5,7) {1};
    \node[fill=selView!12,text=selView!80!black,rounded corners=0.6pt,inner sep=0.25pt,anchor=west,align=center] at (5.50,7.00) {\textbf{selected}\\(correct)};
    \draw[-{Latex[length=2.25mm]},black!75,line width=0.95pt]
      (5,7-\boxSq) -- (5,5.75);
    
    % Image 3 at (3,5), arrow goes RIGHT (toward larger x)
    \path[viewone] (3-\boxSq,5-\boxSq) rectangle (3+\boxSq,5+\boxSq);
    \node[viewnum] at (3,5) {2};
    \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt]
      (3+\boxSq,5) -- (4.25,5);
    
    % Image 4 at (5,3), arrow goes DOWN (toward larger y)
    \path[viewone] (5-\boxSq,3-\boxSq) rectangle (5+\boxSq,3+\boxSq);
    \node[viewnum] at (5,3) {3};
    \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt]
      (5,3+\boxSq) -- (5,4.25);
    
    % Image 1 at (7,5), arrow goes LEFT (toward smaller x)
    \path[viewone] (7-\boxSq,5-\boxSq) rectangle (7+\boxSq,5+\boxSq);
    \node[viewnum] at (7,5) {4};
    \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt]
      (7-\boxSq,5) -- (5.75,5);
    
  
    % ----- Tiny ego-direction compass near selected view -----
    % Facing right: F=+x, B=-x, L=-y, R=+y in map coordinates
    \coordinate (egoC) at (9.00,9.00);
    \fill[selView] (egoC) circle (0.05);
    \draw[-{Latex[length=1.4mm]},line width=0.55pt] (egoC) -- ++(0.36,0);
    \draw[-{Latex[length=1.4mm]},line width=0.55pt] (egoC) -- ++(-0.36,0);
    \draw[-{Latex[length=1.4mm]},line width=0.55pt] (egoC) -- ++(0,-0.36);
    \draw[-{Latex[length=1.4mm]},line width=0.55pt] (egoC) -- ++(0,0.36);
    \node[anchor=west]  at ($(egoC)+(0.25,0)$) {R};
    \node[anchor=east]  at ($(egoC)+(-0.25,0)$) {L};
    \node[anchor=south] at ($(egoC)+(0,-0.2)$) {F};
    \node[anchor=north] at ($(egoC)+(0,0.2)$) {B};
  \end{scope}
\end{tikzpicture}


% % 10x10 cognitive map for among_group458_q1_5_1 (compact + decluttered style)
% \begin{tikzpicture}[font=\fontsize{5.4}{6.0}\selectfont\sffamily]
%   % [0,0] at top-left, y increases downward
%   \begin{scope}[x=0.46cm,y=-0.46cm]
%     % Grid lines
%     \foreach \x in {0,...,10} {\draw[gray!40,line width=0.28pt] (\x,0) -- (\x,10);}
%     \foreach \y in {0,...,10} {\draw[gray!40,line width=0.28pt] (0,\y) -- (10,\y);}
%     \draw[black,line width=0.75pt] (0,0) rectangle (10,10);

%     % Minimal axis ticks (every 2 cells)
%     % \foreach \x in {0,2,4,6,8} {\node[anchor=north] at (\x,10.16) {\x};}
%     % \foreach \y in {0,2,4,6,8} {\node[anchor=east] at (-0.16,\y) {\y};}

%     % Colors for selected-view ego direction
%     \definecolor{selView}{RGB}{210,76,58}
%     \definecolor{egoF}{RGB}{216,68,55}
%     \definecolor{egoB}{RGB}{64,110,185}
%     \definecolor{egoL}{RGB}{226,140,28}
%     \definecolor{egoR}{RGB}{44,158,78}

%     % Styles
%     \tikzset{
%       objdot/.style={draw=black!60,line width=0.35pt,circle,minimum size=4.4pt,inner sep=0pt},
%       objlabel/.style={draw=black!45,fill=white,rounded corners=1.0pt,inner sep=1.0pt,align=center},
%       callout/.style={black!55,line width=0.34pt}
%     }

%     % ----- Object points -----
%     \node[objdot,fill=red!65]         (objBottle) at (5,5) {};
%     \node[objdot,fill=green!60!black] (objCloset) at (5,8) {};
%     \node[objdot,fill=gray!65]        (objWall)   at (2,5) {};
%     \node[objdot,fill=blue!65]        (objWindow) at (4,2) {};
%     \node[objdot,fill=violet!75]      (objPlush)  at (8,5) {};

%     % Label anchor coordinates
%     \coordinate (labWallPos)   at (1.05,4.20);
%     \coordinate (labBottlePos) at (3.55,6.92);
%     \coordinate (labClosetPos) at (5.00,9.08);
%     \coordinate (labWindowPos) at (4.00,1.00);
%     \coordinate (labPlushPos)  at (8.52,3.88);

%     % ----- Callout lines first (to be hidden under white label boxes) -----
%     \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labWallPos) -- (objWall.center);
%     \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labBottlePos) -- (objBottle.center);
%     \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labClosetPos) -- (objCloset.center);
%     \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labWindowPos) -- (objWindow.center);
%     \draw[callout,shorten <=0.6pt,shorten >=0.8pt] (labPlushPos) -- (objPlush.center);

%     % ----- Object labels -----
%     \node[objlabel] at (labWallPos) {white wall\\{\textcolor{egoB}{(back)}}};
%     \node[objlabel] at (labBottlePos) {pink\\bottle\\{\textcolor{egoF}{(forward)}}};
%     \node[objlabel] at (labClosetPos) {closet and door\\(\textcolor{egoF}{forward}-\textcolor{egoR}{right})};
%     \node[objlabel] at (labWindowPos) {window and blue curtain\\(\textcolor{egoL}{left})};
%     \node[objlabel] at (labPlushPos) {pink plush toy\\and headboard\\{\textcolor{egoF}{(forward)}}};

%     % ----- Views: arrows only (selected view highlighted) -----
%     % I1 at (5,6), facing up
%     \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt] (5,6) -- (5,5.25);
%     \node[fill=white,inner sep=0.25pt,anchor=west] at (5.28,6.28) {Image 1};

%     % I2 at (4,5), facing right (selected)
%     \fill[selView] (4,5) circle (0.08);
%     \draw[-{Latex[length=2.25mm]},selView,line width=0.95pt] (4,5) -- (4.78,5);
%     \node[fill=selView!12,text=selView!80!black,rounded corners=0.6pt,inner sep=0.25pt,anchor=west,align=center] at (3.28,3.98) {\textbf{Image 2}\\selected};

%     % I3 at (5,4), facing down
%     \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt] (5,4) -- (5,4.75);
%     \node[fill=white,inner sep=0.25pt,anchor=west] at (5.22,3.72) {Image 3};

%     % I4 at (6,5), facing left
%     \draw[-{Latex[length=2.05mm]},black!75,line width=0.75pt] (6,5) -- (5.25,5);
%     \node[fill=white,inner sep=0.25pt,anchor=west] at (6.22,5.02) {Image 4};

%     % ----- Tiny ego-direction compass near selected view -----
%     % Facing right: F=+x, B=-x, L=-y, R=+y in map coordinates
%     \coordinate (egoC) at (3.05,5.00);
%     \fill[selView] (egoC) circle (0.05);
%     \draw[-{Latex[length=1.4mm]},egoF,line width=0.55pt] (egoC) -- ++(0.36,0);
%     \draw[-{Latex[length=1.4mm]},egoB,line width=0.55pt] (egoC) -- ++(-0.36,0);
%     \draw[-{Latex[length=1.4mm]},egoL,line width=0.55pt] (egoC) -- ++(0,-0.36);
%     \draw[-{Latex[length=1.4mm]},egoR,line width=0.55pt] (egoC) -- ++(0,0.36);
%     \node[anchor=west,text=egoF]  at ($(egoC)+(0.25,0)$) {F};
%     \node[anchor=east,text=egoB]  at ($(egoC)+(-0.25,0)$) {B};
%     \node[anchor=south,text=egoL] at ($(egoC)+(0,-0.2)$) {L};
%     \node[anchor=north,text=egoR] at ($(egoC)+(0,0.2)$) {R};
%   \end{scope}
% \end{tikzpicture}

==> figures/figure_03_04_comb.tex <==

\newcommand{\mvimg}[2]{%
    \begin{tikzpicture}
        \node[inner sep=0, outer sep=0] (img)
        {\includegraphics[width=\linewidth,clip,trim={0 85 0 85}]{#1}};
        \path[use as bounding box] (img.south west) rectangle (img.north east);
        \node[
            anchor=north west,
            fill=white,
            fill opacity=0.88,
            text opacity=1,
            inner sep=0.7pt,
            % font=\fontsize{6.0}{6.0}\selectfont\sffamily\bfseries
            font=\fontsize{17.0}{19.0}\selectfont\sffamily\bfseries
        ] at ([xshift=1pt,yshift=-1pt]img.north west) {#2};
    \end{tikzpicture}%
}

\begin{figure}[t]
    \centering

    \newlength{\qualTopA}
    \newlength{\qualTopB}
    \newlength{\qualTopC}
    \newlength{\qualTopH}
    \newlength{\qualCapH}
    \newlength{\qualImgH}

    \setlength{\qualTopA}{0.31\linewidth}
    \setlength{\qualTopB}{0.27\linewidth}
    \setlength{\qualTopC}{0.36\linewidth}
    % \setlength{\qualTopH}{0.34\textwidth}
    % \setlength{\qualTopH}{0.30\textwidth}  % 03.05 21:00 warning 제거용
    \setlength{\qualTopH}{0.29\textwidth}  % 03.05 21:00 warning 제거용
    \setlength{\qualTopH}{0.25\textwidth}  % 03.06 04:00 페이지 (계속 마지막으로 감)
    \setlength{\qualCapH}{1.8em}
    \setlength{\qualImgH}{\dimexpr\qualTopH-\qualCapH\relax}

    % =========================
    % Example 1
    % =========================
    \begin{tcolorbox}[
        width=\linewidth,
        colback=black!1,
        colframe=black!70,
        boxrule=0.6pt,
        arc=1.2pt,
        after skip=0pt,
        left=1.5mm,right=1.5mm,top=1.1mm,bottom=1.1mm,
        title=\textcolor{white}{\texttt{\textbf{\scriptsize among\_group646\_q0\_2\_1 (MindCube)}}},
        fonttitle=\sffamily\bfseries,
        coltitle=black
    ]

        % ---- top row ----
        \makebox[\linewidth][c]{%
            % (a) Multi-view images
            \begin{minipage}[t][\qualTopH][t]{\qualTopA}
            \centering
        
            \begin{minipage}[c][\qualImgH][c]{\linewidth}
                \centering
                \setlength{\tabcolsep}{0pt}
                \renewcommand{\arraystretch}{0}
                \adjustbox{max width=0.98\linewidth, max totalheight=\qualImgH, keepaspectratio}{%
                    \begin{tabular}{@{}cc@{}}
                        \mvimg{assets/images/among_group646_q0_2_1/front_277.jpg}{1} &  % (Forward)
                        \mvimg{assets/images/among_group646_q0_2_1/left_061.jpg}{2} \\
                        \mvimg{assets/images/among_group646_q0_2_1/back_129.jpg}{3} &
                        \mvimg{assets/images/among_group646_q0_2_1/right_201.jpg}{4}
                    \end{tabular}
                }
            \end{minipage}
        
            \begin{minipage}[b][\qualCapH][c]{\linewidth}
                \centering
                {\tiny (a) Multi-view images}
            \end{minipage}
        \end{minipage}\hfill

            \begin{minipage}[t][\qualTopH][t]{\qualTopB}
                \centering
                \begin{minipage}[c][\qualImgH][c]{\linewidth}
                    \centering
                    \adjustbox{max width=0.98\linewidth, max totalheight=\qualImgH, keepaspectratio}{%
                        \includegraphics[trim={6 6 6 6},clip]{assets/scene/among_group646_scene.pdf}%
                    }
                \end{minipage}

                \begin{minipage}[b][\qualCapH][c]{\linewidth}
                    \centering
                    {\tiny (b) Scene from VFM}
                \end{minipage}
            \end{minipage}\hfill
            % (c) Cognitive map
            \begin{minipage}[t][\qualTopH][t]{\qualTopC}
                \centering
                \begin{minipage}[c][\qualImgH][c]{\linewidth}
                    \centering
                    \adjustbox{max width=0.97\linewidth, max totalheight=\qualImgH, keepaspectratio}{%
                        \input{assets/cogmap/GT/among_group646_q0_2_1_cogmap_tikz.tex}%
                    }
                \end{minipage}

                \begin{minipage}[b][\qualCapH][c]{\linewidth}
                    \centering
                    {\tiny (c) Cognitive map with ego-directions}
                \end{minipage}
            \end{minipage}%
        }

        \par\smallskip

        % ---- text boxes ----
        \begin{tcolorbox}[
            width=\linewidth,
            colback=black!2,
            colframe=black!55,
            boxrule=0.45pt,
            arc=0.9pt,
            before skip=1pt,
            after skip=5pt,
            left=1.1mm,right=1.1mm,top=0.5mm,bottom=0.5mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{Question:} If I am standing at the same spot and facing the same direction as shown in Image~1, what is behind me? \\
        \textbf{Choices:} \textbf{A. Window (GT)} \quad B. Lots of toys \quad C. Wall \quad D. Printed glass door
        \end{tcolorbox}

        \begin{tcolorbox}[
            width=\linewidth,
            colback=red!3,
            colframe=red!70!black,
            boxrule=0.45pt,
            arc=0.9pt,
            left=1.1mm,right=1.1mm,top=0.5mm,bottom=0.5mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{MindCube-SFT:} \texttt{<think>} \; \dots \; The opposite view of the first view is the third view. As ``printed glass door'' is observed behind ``toy helicopter'' in the third view, it means that in the first view, ``printed glass door'' is positioned behind me. \; \dots \; So the answer is \textbf{\textcolor{red!75!black}{``D. Printed glass door''}}. \texttt{</think>}
        \end{tcolorbox}

        \begin{tcolorbox}[
            width=\linewidth,
            colback=green!4,
            colframe=green!45!black,
            boxrule=0.45pt,
            arc=0.9pt,
            left=1.1mm,right=1.1mm,top=0.5mm,bottom=0.5mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{Ours:} \texttt{<think>} \textbf{(1) Selecting a view}: The question uses \textbf{\underline{Image 1}}, so we should consider the viewpoint at \textbf{\underline{Image 1}}. \textbf{(2) Egocentric layout}: The asked direction is ``behind''. In the egomap, ``Window'' has \texttt{ego\_direction}$=$\texttt{``back''}, so it matches ``behind''. \textbf{(3) Confirming in \underline{Image 3}}: ``Window'' can be checked in Image 3. The direction decision comes from the egomap \texttt{ego\_direction} for the asked viewpoint. \textbf{(4)} Therefore, the answer is \textbf{\textcolor{green!25!black}{``A. Window''}}. \texttt{</think>}
        \end{tcolorbox}

    \end{tcolorbox}

    \par\medskip

    % =========================
    % Example 2 (copy-paste block; edit contents later)
    % =========================
    \begin{tcolorbox}[
        width=\linewidth,
        colback=black!1,
        colframe=black!70,
        boxrule=0.6pt,
        arc=1.2pt,
        before skip=0pt,
        after skip=3pt,
        left=1.5mm,right=1.5mm,top=1.1mm,bottom=1.1mm,
        title=\textcolor{white}{\texttt{\textbf{\scriptsize rotation\_group005\_q2\_3 (MindCube)}}},
        fonttitle=\sffamily\bfseries,
        coltitle=black
    ]

        % ---- top row ----
        \makebox[\linewidth][c]{%
            % (a) Multi-view images
            \begin{minipage}[t][\qualTopH][t]{\qualTopA}
            \centering
        
            \begin{minipage}[c][\qualImgH][c]{\linewidth}
                \centering
                \setlength{\tabcolsep}{0pt}
                \renewcommand{\arraystretch}{0}
                \adjustbox{max width=0.98\linewidth, max totalheight=\qualImgH, keepaspectratio}{%
                    \begin{tabular}{@{}cc@{}}
                        \mvimg{assets/images/rotation_group005_q2_3/16.png}{1} &
                        \mvimg{assets/images/rotation_group005_q2_3/28.png}{2} \\  % (Forward)
                        \mvimg{assets/images/rotation_group005_q2_3/40.png}{3}
                    \end{tabular}
                }
            \end{minipage}
        
            \begin{minipage}[b][\qualCapH][c]{\linewidth}
                \centering
                {\tiny (a) Multi-view images}
            \end{minipage}
        \end{minipage}\hfill

            \begin{minipage}[t][\qualTopH][t]{\qualTopB}
                \centering
                \begin{minipage}[c][\qualImgH][c]{\linewidth}
                    \centering
                    \adjustbox{max width=0.98\linewidth, max totalheight=\qualImgH, keepaspectratio}{%
                        \includegraphics[trim={6 6 6 6},clip]{assets/scene/rotation_group005_scene.pdf}%
                    }
                \end{minipage}

                \begin{minipage}[b][\qualCapH][c]{\linewidth}
                    \centering
                    {\tiny (b) Scene from VFM}
                \end{minipage}
            \end{minipage}\hfill
            % (c) Cognitive map
            \begin{minipage}[t][\qualTopH][t]{\qualTopC}
                \centering
                \begin{minipage}[c][\qualImgH][c]{\linewidth}
                    \centering
                    \adjustbox{max width=0.97\linewidth, max totalheight=\qualImgH, keepaspectratio}{%
                        \input{assets/cogmap/GT/rotation_group005_q2_3_cogmap_tikz}%
                    }
                \end{minipage}

                \begin{minipage}[b][\qualCapH][c]{\linewidth}
                    \centering
                    {\tiny (c) Cognitive map with ego-directions}
                \end{minipage}
            \end{minipage}%
        }

        \par\smallskip

        % ---- text boxes ----
        \begin{tcolorbox}[
            width=\linewidth,
            colback=black!2,
            colframe=black!55,
            boxrule=0.45pt,
            arc=0.9pt,
            before skip=1pt,
            after skip=5pt,
            left=1.1mm,right=1.1mm,top=0.5mm,bottom=0.5mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{Question:} If I am standing at the same spot and facing the same direction as shown in image 2, then I turn 90 degrees to the left, what is to my right? \\
        \textbf{Choices:} A. Study table and black chair \quad B. Bed \quad \textbf{C. Window}
        \end{tcolorbox}

        \begin{tcolorbox}[
            width=\linewidth,
            colback=red!3,
            colframe=red!70!black,
            boxrule=0.45pt,
            arc=0.9pt,
            left=1.1mm,right=1.1mm,top=0.5mm,bottom=0.5mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{MindCube-SFT:} \texttt{<think>} \; \dots \; From the perspective of image 2: 'bed' is in front, 'window' is to the right, 'study table and black chair' is behind. After turning 90 degrees to the left: 'window' is now to my right, 'study table and black chair' is now behind me. \; \dots \; So the answer is \textbf{\textcolor{red!75!black}{``B. Bed''}}. \texttt{</think>}
        \end{tcolorbox}

        \begin{tcolorbox}[
            width=\linewidth,
            colback=green!4,
            colframe=green!45!black,
            boxrule=0.45pt,
            arc=0.9pt,
            left=1.1mm,right=1.1mm,top=0.5mm,bottom=0.5mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{Ours:} \texttt{<think>} \textbf{(1) Selecting a view}: After turning ``left'' from Image 2, it corresponds to the facing direction of \textbf{\underline{Image 1}}, so we should consider the viewpoint at \textbf{\underline{Image 1}}. \textbf{(2) Egocentric layout}: The asked direction is ``right''. In the egomap, ``Window'' has \texttt{ego\_direction}$=$\texttt{``right''}, so it matches ``right''. \textbf{(3) Confirming in \underline{Image 2}}: ``Window'' can be checked in Image 2. \textbf{(4)} Therefore, the answer is \textbf{\textcolor{green!25!black}{``C. Window''}}. \texttt{</think>}
        \end{tcolorbox}

    \end{tcolorbox}
    \caption{\textbf{Qualitative comparison.} Top: multi-view inputs and a cognitive map with ego-direction cues from our model (Qwen 2.5-VL-3B-Instruct) trained with SFT and GRPO. Bottom: question prompt and reasoning excerpts. The baseline confuses spatial directions and predicts the wrong object, whereas our method reasons over egocentric directions step by step and predicts the correct object in this example.}
    \label{fig:quali_mindcube}
\end{figure}



==> figures/figure_05.tex <==



% ---- length declarations (before using \setlength) ----

\newcommand{\mvimgTwo}[2]{%
    \begin{tikzpicture}
        \node[inner sep=0, outer sep=0] (img)
        {\includegraphics[width=\linewidth,clip,trim={0 0 0 0}]{#1}};
        \path[use as bounding box] (img.south west) rectangle (img.north east);
        \node[
            anchor=north west,
            fill=white,
            fill opacity=0.88,
            text opacity=1,
            inner sep=0.7pt,
            % font=\fontsize{6.0}{6.0}\selectfont\sffamily\bfseries
            font=\fontsize{17.0}{19.0}\selectfont\sffamily\bfseries
        ] at ([xshift=1pt,yshift=-1pt]img.north west) {#2};
    \end{tikzpicture}%
}

\begin{figure}[t]
    \centering

    % ---- layout params ----
    \setlength{\qualTopA}{0.58\linewidth} % (a) wide
    \setlength{\qualTopB}{0.40\linewidth} % (b) cogmap
    \setlength{\qualTopH}{0.27\textwidth} % adjust as needed
    \setlength{\qualCapH}{1.7em}
    \setlength{\qualImgH}{\dimexpr\qualTopH-\qualCapH\relax}

    \begin{tcolorbox}[
        width=\linewidth,
        colback=black!1,
        colframe=black!70,
        boxrule=0.6pt,
        arc=1.2pt,
        before skip=0pt,
        after skip=3pt,
        left=1.5mm,right=1.5mm,top=1.1mm,bottom=1.1mm,
        title=\textcolor{white}{\texttt{\textbf{\scriptsize route\_planning\_38d58a7a31 (VSI-Bench)}}}, % e.g., scannetpp_d755b3d9d8
        fonttitle=\sffamily\bfseries,
        coltitle=black
    ]

        % =========================
        % (a) Multi-view images (8 images, 4x2)
        % =========================
        \makebox[\linewidth][c]{%
            \begin{minipage}[t][\qualTopH][t]{\qualTopA}
                \centering
                \begin{minipage}[c][\qualImgH][c]{\linewidth}
                    \centering
                    \setlength{\tabcolsep}{1.0pt}
                    \renewcommand{\arraystretch}{0}
                    \adjustbox{max width=0.99\linewidth, max totalheight=\qualImgH, keepaspectratio}{%
                        \begin{tabular}{@{}cccc@{}}
                            \mvimgTwo{assets/images/route_planning_38d58a7a31/ex1_d755b3d9d8_frame0.jpg}{1} &
                            \mvimgTwo{assets/images/route_planning_38d58a7a31/ex1_d755b3d9d8_frame1.jpg}{2} &
                            \mvimgTwo{assets/images/route_planning_38d58a7a31/ex1_d755b3d9d8_frame2.jpg}{3} &
                            \mvimgTwo{assets/images/route_planning_38d58a7a31/ex1_d755b3d9d8_frame3.jpg}{4} \\
                            \mvimgTwo{assets/images/route_planning_38d58a7a31/ex1_d755b3d9d8_frame4.jpg}{5} &
                            \mvimgTwo{assets/images/route_planning_38d58a7a31/ex1_d755b3d9d8_frame5.jpg}{6} &
                            \mvimgTwo{assets/images/route_planning_38d58a7a31/ex1_d755b3d9d8_frame6.jpg}{7} &
                            \mvimgTwo{assets/images/route_planning_38d58a7a31/ex1_d755b3d9d8_frame7.jpg}{8}
                        \end{tabular}
                    }
                \end{minipage}

                \begin{minipage}[b][\qualCapH][c]{\linewidth}
                    \centering
                    {\tiny (a) Multi-frame video}
                \end{minipage}
            \end{minipage}\hfill
            % =========================
            % (b) Cogmap
            % =========================
            \begin{minipage}[t][\qualTopH][t]{\qualTopB}
                \centering
                \begin{minipage}[c][\qualImgH][c]{\linewidth}
                    \centering
                    \adjustbox{max width=0.98\linewidth, max totalheight=\qualImgH, keepaspectratio}{%
                        \input{assets/cogmap/MLLM/route_planning_38d58a7a31_cogmap_tikz}%
                    }
                \end{minipage}

                \begin{minipage}[b][\qualCapH][c]{\linewidth}
                    \centering
                    {\tiny (b) CogMap with ego-directions}
                \end{minipage}
            \end{minipage}%
        }

        \par\smallskip



        % =========================
        % Text boxes: Question + Ours only
        % =========================
        \begin{tcolorbox}[
            width=\linewidth,
            colback=black!2,
            colframe=black!55,
            boxrule=0.45pt,
            arc=0.9pt,
            before skip=1pt,
            after skip=2pt,
            left=1.1mm,right=1.1mm,top=0.5mm,bottom=0.5mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{Question:} If I am standing by the door and facing the cup, is the whiteboard to my left, right, or back? \\
        \textbf{Choices:} \textbf{A. left (GT)} \quad B. back \quad C. right
        \end{tcolorbox}

        \begin{tcolorbox}[
            width=\linewidth,
            colback=red!2,
            colframe=red!65!black,
            boxrule=0.40pt,
            arc=0.9pt,
            before skip=2pt,
            after skip=2pt,
            left=1.1mm,right=1.1mm,top=0.45mm,bottom=0.45mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{Other models:}\; {\color{red!75!black}\xmark}\;LLaVA-NeXT \textcolor{red!75!black}{(C. right)} \qquad
        {\color{red!75!black}\xmark}\;LLaVA-OV \textcolor{red!75!black}{(B. back)} \qquad
        {\color{red!75!black}\xmark}\;VILA \textcolor{red!75!black}{(B. back)}
        \end{tcolorbox}

        \begin{tcolorbox}[
            width=\linewidth,
            colback=green!4,
            colframe=green!45!black,
            boxrule=0.45pt,
            arc=0.9pt,
            before skip=2pt,
            after skip=2pt,
            left=1.1mm,right=1.1mm,top=0.5mm,bottom=0.5mm,
            fontupper=\fontsize{6}{7}\selectfont\sffamily
        ]
        \textbf{Ours:} \texttt{<think>} 
        \textbf{(1) Selecting a viewpoint}: According to the CogMap, the door is at (5,5). The question asks: ``standing by the door and facing the cup'' \dots which point diagonally toward the \underline{\textbf{top-right}} in the CogMap. \textbf{(2) Egocentric layout}: From the door's position (5,5), facing toward the cup (7,3):
        \dots Compared to the facing direction (+2,-2), the whiteboard direction (0,-2) is rotated to the left side of the viewer's frame under this facing direction. This corresponds to ``left.'' \textbf{(3) Confirming}: \dots When facing toward the top-right (toward the cup), this places the whiteboard in the front-left region of the ego frame, matching the ``left'' choice.
        \textbf{(4)} Therefore, the answer is \textbf{\textcolor{green!25!black}{``A. left''}}. 
        \texttt{</think>}
        \end{tcolorbox}

    \end{tcolorbox}

    \caption{
        \textbf{Qualitative example on VSI-Bench (video).}
        Although trained only on static multi-view images, our model generalizes to video input by constructing a coherent cognitive map and performing egocentric spatial reasoning with sampled frames.
    }
    \label{fig:quali_vsi_bench}
    % \vspace{-15pt}
\end{figure}

==> rebuttal_cvpr_org.tex <==
% ---------------------------------------------------------------
%
% No guarantee is given that the format corresponds perfectly to
% IEEE 8.5" x 11" Proceedings, but most features should be ok.
%
% ---------------------------------------------------------------
% with LaTeX2e:
% =============
%
% use as
%   \documentclass[times,10pt,twocolumn]{article}
%   \usepackage[options]{cvpr}
%   \usepackage{times}
%
% "options" should be replaced by
%  * "review" for submitting a paper for review,
%  * "final" for the camera ready, and
%  * "rebuttal" for the author rebuttal.
%
% specify references as
%   {\small
%   \bibliographystyle{ieee}
%   \bibliography{...your files...}
%   }
% ---------------------------------------------------------------

\NeedsTeXFormat{LaTeX2e}[1999/12/01]
\ProvidesPackage{cvpr}[2024 Example LaTex class for IEEE CVPR]

\RequirePackage{times}    % Integrate Times for here
\RequirePackage{xspace}
\RequirePackage[dvipsnames]{xcolor}
\RequirePackage{graphicx}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{booktabs}
\RequirePackage[numbers,sort&compress]{natbib}
\setlength{\bibsep}{1pt plus 1pt minus 1pt}

\RequirePackage{silence}  % Suppress unwanted warnings
\hbadness=10000 \vbadness=10000 \vfuzz=30pt \hfuzz=30pt
\WarningFilter{latexfont}{Font shape declaration}
\WarningFilter{latex}{Font shape}
\WarningFilter{hyperref}{Token not allowed in a PDF string}
\WarningFilter[rebuttal]{latex}{No \author given}
\RequirePackage{etoolbox}

% Use modern caption package to allow for sub-figures etc.
% Reproduces the original CVPR/ICCV style as closely as possible.
\RequirePackage[format=plain,labelformat=simple,labelsep=period,font=small,tableposition=bottom]{caption}
\RequirePackage[font=footnotesize,skip=3pt,subrefformat=parens]{subcaption}


\newtoggle{cvprfinal}        % Camera-ready version
\newtoggle{cvprrebuttal}     % Rebuttal
\newtoggle{cvprpagenumbers}  % Force page numbers (in camera ready)
\toggletrue{cvprfinal}
\togglefalse{cvprrebuttal}
\togglefalse{cvprpagenumbers}
\DeclareOption{review}{\togglefalse{cvprfinal}\toggletrue{cvprpagenumbers}}
\DeclareOption{rebuttal}{\togglefalse{cvprfinal}\toggletrue{cvprrebuttal}}
\DeclareOption{pagenumbers}{\toggletrue{cvprpagenumbers}}
\DeclareOption*{\PackageWarning{cvpr}{Unkown option `\CurrentOption'}}
\ProcessOptions\relax

% Don't warn about missing author for rebuttal
\iftoggle{cvprrebuttal}{%
  \ActivateWarningFilters[rebuttal]
}{}

% Breaking lines for URLs in the bib
\RequirePackage[hyphens]{url}
\Urlmuskip=0mu plus 1mu\relax


% ---------------------------------------------------------------
\newcommand{\@EveryShipout@Hook}{}
\newcommand{\@EveryShipout@AtNextHook}{}
\newcommand*{\EveryShipout}[1]
   {\g@addto@macro\@EveryShipout@Hook{#1}}
\newcommand*{\AtNextShipout}[1]
   {\g@addto@macro\@EveryShipout@AtNextHook{#1}}
\newcommand{\@EveryShipout@Shipout}{%
   \afterassignment\@EveryShipout@Test
   \global\setbox\@cclv= %
   }
\newcommand{\@EveryShipout@Test}{%
   \ifvoid\@cclv\relax
      \aftergroup\@EveryShipout@Output
   \else
      \@EveryShipout@Output
   \fi%
   }
\newcommand{\@EveryShipout@Output}{%
   \@EveryShipout@Hook%
   \@EveryShipout@AtNextHook%
      \gdef\@EveryShipout@AtNextHook{}%
   \@EveryShipout@Org@Shipout\box\@cclv%
   }
\newcommand{\@EveryShipout@Org@Shipout}{}
\newcommand*{\@EveryShipout@Init}{%
   \message{ABD: EveryShipout initializing macros}%
   \let\@EveryShipout@Org@Shipout\shipout
   \let\shipout\@EveryShipout@Shipout
   }
\AtBeginDocument{\@EveryShipout@Init}

% ---------------------------------------------------------------



\newcommand\LenToUnit[1]{#1\@gobble}

\newcommand\AtPageUpperLeft[1]{%
  \begingroup
    \@tempdima=0pt\relax\@tempdimb=\ESO@yoffsetI\relax
    \put(\LenToUnit{\@tempdima},\LenToUnit{\@tempdimb}){#1}%
  \endgroup
}
\newcommand\AtPageLowerLeft[1]{\AtPageUpperLeft{%
  \put(0,\LenToUnit{-\paperheight}){#1}}}
\newcommand\AtPageCenter[1]{\AtPageUpperLeft{%
  \put(\LenToUnit{.5\paperwidth},\LenToUnit{-.5\paperheight}){#1}}%
}
\newcommand\AtTextUpperLeft[1]{%
  \begingroup
    \setlength\@tempdima{1in}%
    \ifodd\c@page%
      \advance\@tempdima\oddsidemargin%
    \else%
      \advance\@tempdima\evensidemargin%
    \fi%
    \@tempdimb=\ESO@yoffsetI\relax\advance\@tempdimb-1in\relax%
    \advance\@tempdimb-\topmargin%
    \advance\@tempdimb-\headheight\advance\@tempdimb-\headsep%
    \put(\LenToUnit{\@tempdima},\LenToUnit{\@tempdimb}){#1}%
  \endgroup
}
\newcommand\AtTextLowerLeft[1]{\AtTextUpperLeft{%
  \put(0,\LenToUnit{-\textheight}){#1}}}
\newcommand\AtTextCenter[1]{\AtTextUpperLeft{%
  \put(\LenToUnit{.5\textwidth},\LenToUnit{-.5\textheight}){#1}}}
\newcommand{\ESO@HookI}{} \newcommand{\ESO@HookII}{}
\newcommand{\ESO@HookIII}{}
\newcommand{\AddToShipoutPicture}{%
  \@ifstar{\g@addto@macro\ESO@HookII}{\g@addto@macro\ESO@HookI}}
\newcommand{\ClearShipoutPicture}{\global\let\ESO@HookI\@empty}
\newcommand\ESO@isMEMOIR[1]{}
\@ifclassloaded{memoir}{\renewcommand\ESO@isMEMOIR[1]{#1}}{}
\newcommand{\@ShipoutPicture}{%
  \bgroup
    \@tempswafalse%
    \ifx\ESO@HookI\@empty\else\@tempswatrue\fi%
    \ifx\ESO@HookII\@empty\else\@tempswatrue\fi%
    \ifx\ESO@HookIII\@empty\else\@tempswatrue\fi%
    \if@tempswa%
      \@tempdima=1in\@tempdimb=-\@tempdima%
      \advance\@tempdimb\ESO@yoffsetI%
      \ESO@isMEMOIR{%
        \advance\@tempdima\trimedge%
        \advance\@tempdima\paperwidth%
        \advance\@tempdima-\stockwidth%
        \if@twoside\ifodd\c@page\else%
          \advance\@tempdima-2\trimedge%
          \advance\@tempdima-\paperwidth%
          \advance\@tempdima\stockwidth%
        \fi\fi%
        \advance\@tempdimb\trimtop}%
      \unitlength=1pt%
      \global\setbox\@cclv\vbox{%
        \vbox{\let\protect\relax
          \pictur@(0,0)(\strip@pt\@tempdima,\strip@pt\@tempdimb)%
            \ESO@HookIII\ESO@HookI\ESO@HookII%
            \global\let\ESO@HookII\@empty%
          \endpicture}%
          \nointerlineskip%
        \box\@cclv}%
    \fi
  \egroup
}
\EveryShipout{\@ShipoutPicture}
\RequirePackage{keyval}
\newif\ifESO@dvips\ESO@dvipsfalse \newif\ifESO@grid\ESO@gridfalse
\newif\ifESO@texcoord\ESO@texcoordfalse
\newcommand*\ESO@gridunitname{}
\newcommand*\ESO@gridunit{}
\newcommand*\ESO@labelfactor{}
\newcommand*\ESO@griddelta{}\newcommand*\ESO@griddeltaY{}
\newcommand*\ESO@gridDelta{}\newcommand*\ESO@gridDeltaY{}
\newcommand*\ESO@gridcolor{}
\newcommand*\ESO@subgridcolor{}
\newcommand*\ESO@subgridstyle{dotted}% ???
\newcommand*\ESO@gap{}
\newcommand*\ESO@yoffsetI{}\newcommand*\ESO@yoffsetII{}
\newcommand*\ESO@gridlines{\thinlines}
\newcommand*\ESO@subgridlines{\thinlines}
\newcommand*\ESO@hline[1]{\ESO@subgridlines\line(1,0){#1}}
\newcommand*\ESO@vline[1]{\ESO@subgridlines\line(0,1){#1}}
\newcommand*\ESO@Hline[1]{\ESO@gridlines\line(1,0){#1}}
\newcommand*\ESO@Vline[1]{\ESO@gridlines\line(0,1){#1}}
\newcommand\ESO@fcolorbox[4][]{\fbox{#4}}
\newcommand\ESO@color[1]{}
\newcommand\ESO@colorbox[3][]{%
  \begingroup
    \fboxrule=0pt\fbox{#3}%
  \endgroup
}
\newcommand\gridSetup[6][]{%
  \edef\ESO@gridunitname{#1}\edef\ESO@gridunit{#2}
  \edef\ESO@labelfactor{#3}\edef\ESO@griddelta{#4}
  \edef\ESO@gridDelta{#5}\edef\ESO@gap{#6}}
\define@key{ESO}{texcoord}[true]{\csname ESO@texcoord#1\endcsname}
\define@key{ESO}{pscoord}[true]{\csname @tempswa#1\endcsname
  \if@tempswa\ESO@texcoordfalse\else\ESO@texcoordtrue\fi}
\define@key{ESO}{dvips}[true]{\csname ESO@dvips#1\endcsname}
\define@key{ESO}{grid}[true]{\csname ESO@grid#1\endcsname
  \setkeys{ESO}{gridcolor=black,subgridcolor=black}}
\define@key{ESO}{colorgrid}[true]{\csname ESO@grid#1\endcsname
  \setkeys{ESO}{gridcolor=red,subgridcolor=green}}
\define@key{ESO}{gridcolor}{\def\ESO@gridcolor{#1}}
\define@key{ESO}{subgridcolor}{\def\ESO@subgridcolor{#1}}
\define@key{ESO}{subgridstyle}{\def\ESO@subgridstyle{#1}}%
\define@key{ESO}{gridunit}{%
  \def\@tempa{#1}
  \def\@tempb{bp}
  \ifx\@tempa\@tempb
    \gridSetup[\@tempa]{1bp}{1}{10}{50}{2}
  \else
    \def\@tempb{pt}
    \ifx\@tempa\@tempb
      \gridSetup[\@tempa]{1pt}{1}{10}{50}{2}
    \else
      \def\@tempb{in}
      \ifx\@tempa\@tempb
        \gridSetup[\@tempa]{.1in}{.1}{2}{10}{.5}
      \else
        \gridSetup[mm]{1mm}{1}{5}{20}{1}
      \fi
    \fi
  \fi
}


\newcommand\ESO@div[2]{%
  \@tempdima=#1\relax\@tempdimb=\ESO@gridunit\relax
  \@tempdimb=#2\@tempdimb\divide\@tempdima by \@tempdimb%
  \@tempcnta\@tempdima\advance\@tempcnta\@ne}
\AtBeginDocument{%
  \IfFileExists{color.sty}
  {%
    \RequirePackage{color}
    \let\ESO@color=\color\let\ESO@colorbox=\colorbox
    \let\ESO@fcolorbox=\fcolorbox
  }{}
  \@ifundefined{Gin@driver}{}%
  {%
    \ifx\Gin@driver\@empty\else%
      \filename@parse{\Gin@driver}\def\reserved@a{dvips}%
      \ifx\filename@base\reserved@a\ESO@dvipstrue\fi%
    \fi
  }%
  \ifx\pdfoutput\undefined\else
    \ifx\pdfoutput\relax\else
      \ifcase\pdfoutput\else
        \ESO@dvipsfalse%
      \fi
    \fi
  \fi
  \ifESO@dvips\def\@tempb{eepic}\else\def\@tempb{epic}\fi
  \def\@tempa{dotted}%\def\ESO@gap{\LenToUnit{6\@wholewidth}}%
  \ifx\@tempa\ESO@subgridstyle
    \IfFileExists{\@tempb.sty}%
    {%
      \RequirePackage{\@tempb}
      \renewcommand*\ESO@hline[1]{\ESO@subgridlines\dottedline{\ESO@gap}%
        (0,0)(##1,0)}
      \renewcommand*\ESO@vline[1]{\ESO@subgridlines\dottedline{\ESO@gap}%
        (0,0)(0,##1)}
    }{}
  \else
    \ifx\ESO@gridcolor\ESO@subgridcolor%
      \renewcommand*\ESO@gridlines{\thicklines}
    \fi
  \fi
}
\ifESO@texcoord
  \def\ESO@yoffsetI{0pt}\def\ESO@yoffsetII{-\paperheight}
  \edef\ESO@griddeltaY{-\ESO@griddelta}\edef\ESO@gridDeltaY{-\ESO@gridDelta}
\else
  \def\ESO@yoffsetI{\paperheight}\def\ESO@yoffsetII{0pt}
  \edef\ESO@griddeltaY{\ESO@griddelta}\edef\ESO@gridDeltaY{\ESO@gridDelta}
\fi
\newcommand\ESO@gridpicture{%
  \begingroup
    \setlength\unitlength{\ESO@gridunit}%
    \ESO@color{\ESO@subgridcolor}%
    \ESO@div{\paperheight}{\ESO@griddelta}%
    \multiput(0,0)(0,\ESO@griddeltaY){\@tempcnta}%
      {\ESO@hline{\LenToUnit{\paperwidth}}}%
    \ESO@div{\paperwidth}{\ESO@griddelta}%
    \multiput(0,\LenToUnit{\ESO@yoffsetII})(\ESO@griddelta,0){\@tempcnta}%
      {\ESO@vline{\LenToUnit{\paperheight}}}%
    \ESO@color{\ESO@gridcolor}%
    \ESO@div{\paperheight}{\ESO@gridDelta}%
    \multiput(0,0)(0,\ESO@gridDeltaY){\@tempcnta}%
      {\ESO@Hline{\LenToUnit{\paperwidth}}}%
    \ESO@div{\paperwidth}{\ESO@gridDelta}%
    \multiput(0,\LenToUnit{\ESO@yoffsetII})(\ESO@gridDelta,0){\@tempcnta}%
      {\ESO@Vline{\LenToUnit{\paperheight}}}%
    \fontsize{10}{12}\normalfont%
    \ESO@div{\paperwidth}{\ESO@gridDelta}%
    \multiput(0,\ESO@gridDeltaY)(\ESO@gridDelta,0){\@tempcnta}{%
      \@tempcntb=\@tempcnta\advance\@tempcntb-\@multicnt%
      \ifnum\@tempcntb>1\relax
        \multiply\@tempcntb by \ESO@gridDelta\relax%
        \@tempdima=\@tempcntb sp\@tempdima=\ESO@labelfactor\@tempdima%
        \@tempcntb=\@tempdima%
        \makebox(0,0)[c]{\ESO@colorbox{white}{\the\@tempcntb}}%
      \fi}%
    \ifx\ESO@gridunitname\@empty\def\@tempa{0}\else\def\@tempa{1}\fi%
    \ESO@div{\paperheight}{\ESO@gridDelta}%
    \multiput(\ESO@gridDelta,0)(0,\ESO@gridDeltaY){\@tempcnta}{%
      \@tempcntb=\@tempcnta\advance\@tempcntb-\@multicnt%
      \ifnum\@tempcntb>\@tempa\relax
        \multiply\@tempcntb by \ESO@gridDelta\relax%
        \@tempdima=\@tempcntb sp\@tempdima=\ESO@labelfactor\@tempdima%
        \@tempcntb=\@tempdima%
        \makebox(0,0)[c]{\ESO@colorbox{white}{\the\@tempcntb}}%
      \fi
    }%
    \ifx\ESO@gridunitname\@empty\else%
      \thicklines\fboxrule=\@wholewidth%
      \put(\ESO@gridDelta,\ESO@gridDeltaY){\makebox(0,0)[c]{%
        \ESO@fcolorbox{\ESO@gridcolor}{white}{%
          \textbf{\ESO@gridunitname}}}}%
    \fi
    \normalcolor%
  \endgroup
}
\ifESO@grid\g@addto@macro\ESO@HookIII{\ESO@gridpicture}\fi
% ---------------------------------------------------------------




\typeout{CVPR 8.5 x 11-Inch Proceedings Style `cvpr.sty'.}

% ten point helvetica bold required for captions
% eleven point times bold required for second-order headings
% in some sites the name of the fonts may differ,
% change the name here:
\font\cvprtenhv  = phvb at 8pt % *** IF THIS FAILS, SEE cvpr.sty ***
\font\elvbf  = ptmb scaled 1100

% If the above lines give an error message, try to comment them and
% uncomment these:
%\font\cvprtenhv  = phvb7t at 8pt
%\font\elvbf  = ptmb7t scaled 1100

% set dimensions of columns, gap between columns, and paragraph indent
\setlength{\textheight}{8.875in}
\setlength{\textwidth}{6.875in}
\setlength{\columnsep}{0.3125in}
\setlength{\topmargin}{0in}
\setlength{\headheight}{0in}
\setlength{\headsep}{0in}
\setlength{\parindent}{1pc}
\setlength{\oddsidemargin}{-.1875in}
\setlength{\evensidemargin}{-.1875in}


% Suppress page numbers when the appropriate option is given
\iftoggle{cvprpagenumbers}{}{%
  \pagestyle{empty}
}

\AtBeginDocument{%
  % Print an error if document class other than article is used
  \@ifclassloaded{article}{}{%
    \PackageError{cvpr}{Package only meant to be used with document class `article'}{Change document class to `article'.}
  }
  % Print a warning if incorrect options for article are specified
  \@ifclasswith{article}{10pt}{}{%
    \PackageWarningNoLine{cvpr}{Incorrect font size specified - CVPR requires 10-point fonts. Please load document class `article' with `10pt' option}
  }
  \@ifclasswith{article}{twocolumn}{}{%
    \PackageWarningNoLine{cvpr}{Single column document - CVPR requires papers to have two-column layout. Please load document class `article' with `twocolumn' option}
  }
  \@ifclasswith{article}{letterpaper}{}{%
    \PackageWarningNoLine{cvpr}{Incorrect paper size - CVPR uses paper size `letter'. Please load document class `article' with `letterpaper' option}
  }
  % Print a warning if hyperref is not loaded and/or if the pagebackref option is missing
  \iftoggle{cvprfinal}{%
    \@ifpackageloaded{hyperref}{}{%
      \PackageWarningNoLine{cvpr}{Package `hyperref' is not loaded, but highly recommended for camera-ready version}
    }
  }{%
    \@ifpackageloaded{hyperref}{
      \@ifpackagewith{hyperref}{pagebackref}{}{
        \PackageWarningNoLine{cvpr}{Package `hyperref' is not loaded with option `pagebackref', which is strongly recommended for review version}
      }
    }{%
      \PackageWarningNoLine{cvpr}{Package `hyperref' is not loaded, but strongly recommended for review version}
    }
  }
}

\def\@maketitle{
   \newpage
   \null
   \iftoggle{cvprrebuttal}{\vspace*{-.3in}}{\vskip .375in}
   \begin{center}
      % smaller title font only for rebuttal
      \iftoggle{cvprrebuttal}{{\large \bf \@title \par}}{{\Large \bf \@title \par}}
      % additional two empty lines at the end of the title
      \iftoggle{cvprrebuttal}{\vspace*{-22pt}}{\vspace*{24pt}}{
        \large
        \lineskip .5em
        \begin{tabular}[t]{c}
          \iftoggle{cvprfinal}{
            \@author
          }{
            \iftoggle{cvprrebuttal}{}{
              Anonymous \confName~submission\\
              \vspace*{1pt}\\
              Paper ID \paperID
            }
          }
        \end{tabular}
        \par
      }
      % additional small space at the end of the author name
      \vskip .5em
      % additional empty line at the end of the title block
      \vspace*{12pt}
   \end{center}
}

\def\abstract{%
   % Suppress page numbers when the appropriate option is given
   \iftoggle{cvprpagenumbers}{}{%
     \thispagestyle{empty}
   }
   \centerline{\large\bf Abstract}%
   \vspace*{12pt}\noindent%
   \it\ignorespaces%
}

\def\endabstract{%
   % additional empty line at the end of the abstract
   \vspace*{12pt}
   }

\def\affiliation#1{\gdef\@affiliation{#1}} \gdef\@affiliation{}

% correct heading spacing and type
\def\cvprsection{\@startsection {section}{1}{\z@}
   {-10pt plus -2pt minus -2pt}{7pt} {\large\bf}}
\def\cvprssect#1{\cvprsection*{#1}}
\def\cvprsect#1{\cvprsection{\hskip -1em.~#1}}
\def\section{\@ifstar\cvprssect\cvprsect}

\def\cvprsubsection{\@startsection {subsection}{2}{\z@}
   {-8pt plus -2pt minus -2pt}{6pt} {\elvbf}}
\def\cvprssubsect#1{\cvprsubsection*{#1}}
\def\cvprsubsect#1{\cvprsubsection{\hskip -1em.~#1}}
\def\subsection{\@ifstar\cvprssubsect\cvprsubsect}

%% --------- Page background marks: Ruler and confidentiality

% ----- define vruler
\makeatletter
\newbox\cvprrulerbox
\newcount\cvprrulercount
\newdimen\cvprruleroffset
\newdimen\cv@lineheight
\newdimen\cv@boxheight
\newbox\cv@tmpbox
\newcount\cv@refno
\newcount\cv@tot
% NUMBER with left flushed zeros  \fillzeros[<WIDTH>]<NUMBER>
\newcount\cv@tmpc@ \newcount\cv@tmpc
\def\fillzeros[#1]#2{\cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi
\cv@tmpc=1 %
\loop\ifnum\cv@tmpc@<10 \else \divide\cv@tmpc@ by 10 \advance\cv@tmpc by 1 \fi
   \ifnum\cv@tmpc@=10\relax\cv@tmpc@=11\relax\fi \ifnum\cv@tmpc@>10 \repeat
\ifnum#2<0\advance\cv@tmpc1\relax-\fi
\loop\ifnum\cv@tmpc<#1\relax0\advance\cv@tmpc1\relax\fi \ifnum\cv@tmpc<#1 \repeat
\cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi \relax\the\cv@tmpc@}%
\makeatother
% ----- end of vruler

%% Define linenumber setup
\RequirePackage[switch,mathlines]{lineno}

% Line numbers in CVPR blue using font from \cvprtenhv
\renewcommand\linenumberfont{\cvprtenhv\color{eccvblue}}

\renewcommand\thelinenumber{\fillzeros[3]{\arabic{linenumber}}}

\setlength{\linenumbersep}{.75cm}

% Bug: An equation with $$ ... $$ isn't numbered, nor is the previous line.

% Patch amsmath commands so that the previous line and the equation itself
% are numbered. Bug: multiline has an extra line number.
% https://tex.stackexchange.com/questions/461186/how-to-use-lineno-with-amsmath-align
\RequirePackage{etoolbox} %% <- for \pretocmd, \apptocmd and \patchcmd

\newcommand*\linenomathpatch[1]{%
  \expandafter\pretocmd\csname #1\endcsname {\linenomath}{}{}%
  \expandafter\pretocmd\csname #1*\endcsname {\linenomath}{}{}%
  \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}%
  \expandafter\apptocmd\csname end#1*\endcsname {\endlinenomath}{}{}%
}
\newcommand*\linenomathpatchAMS[1]{%
  \expandafter\pretocmd\csname #1\endcsname {\linenomathAMS}{}{}%
  \expandafter\pretocmd\csname #1*\endcsname {\linenomathAMS}{}{}%
  \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}%
  \expandafter\apptocmd\csname end#1*\endcsname {\endlinenomath}{}{}%
}

%% Definition of \linenomathAMS depends on whether the mathlines option is provided
\expandafter\ifx\linenomath\linenomathWithnumbers
\let\linenomathAMS\linenomathWithnumbers
%% The following line gets rid of an extra line numbers at the bottom:
\patchcmd\linenomathAMS{\advance\postdisplaypenalty\linenopenalty}{}{}{}
\else
\let\linenomathAMS\linenomathNonumbers
\fi

\iftoggle{cvprfinal}{}{
% Add the numbers
\linenumbers
\AtBeginDocument{%
  \linenomathpatch{equation}%
  \linenomathpatchAMS{gather}%
  \linenomathpatchAMS{multline}%
  \linenomathpatchAMS{align}%
  \linenomathpatchAMS{alignat}%
  \linenomathpatchAMS{flalign}%
}
}

% \makevruler[<SCALE>][<INITIAL_COUNT>][<STEP>][<DIGITS>][<HEIGHT>]
\def\cvprruler#1{\makevruler[12pt][#1][1][3][0.993\textheight]\usebox{\cvprrulerbox}}
\AddToShipoutPicture{%
  \iftoggle{cvprfinal}{
  }{
    \color{eccvblue}

    \def\pid{\parbox{1in}{\begin{center}\bf\sf{\small \confName}\\\#\paperID\end{center}}}
    \AtTextUpperLeft{%paperID in corners
      \put(\LenToUnit{-65pt},\LenToUnit{45pt}){\pid}
      \put(\LenToUnit{\textwidth\kern-8pt},\LenToUnit{45pt}){\pid}
    }
    \AtTextUpperLeft{%confidential
      \put(0,\LenToUnit{1cm}){\parbox{\textwidth}{\centering\cvprtenhv
      \confName~\confYear~Rebuttal~for~Submission \#\paperID. CONFIDENTIAL REVIEW COPY.  DO NOT DISTRIBUTE.}}
    }
  }
}

%%% Make figure placement a little more predictable.
% We trust the user to move figures if this results
% in ugliness.
% Minimize bad page breaks at figures
\renewcommand{\textfraction}{0.01}
\renewcommand{\floatpagefraction}{0.99}
\renewcommand{\topfraction}{0.99}
\renewcommand{\bottomfraction}{0.99}
\renewcommand{\dblfloatpagefraction}{0.99}
\renewcommand{\dbltopfraction}{0.99}
\setcounter{totalnumber}{99}
\setcounter{topnumber}{99}
\setcounter{bottomnumber}{99}

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

% ---------------------------------------------------------------

%% redefine the \title command so that a variable name is saved in \thetitle, and provides the \maketitlesupplementary command
\let\titleold\title
\renewcommand{\title}[1]{\titleold{#1}\newcommand{\thetitle}{#1}}
\def\maketitlesupplementary
   {
   \newpage
       \twocolumn[
        \centering
        \Large
        \textbf{\thetitle}\\
        \vspace{0.5em}Supplementary Material \\
        \vspace{1.0em}
       ] %< twocolumn
   }

% ---------------------------------------------------------------

%% Support for easy cross-referencing (e.g. \cref{sec:intro}
% configured with \AtEndPreamble as it needs to be called after hyperref
\AtEndPreamble{
    \usepackage[capitalize]{cleveref}
    \crefname{section}{Sec.}{Secs.}
    \Crefname{section}{Section}{Sections}
    \Crefname{table}{Table}{Tables}
    \crefname{table}{Tab.}{Tabs.}
}

% ---------------------------------------------------------------

%% More compact compact itemize/enumeration (e.g. list contributions)
\RequirePackage{enumitem}
\setlist[itemize]{noitemsep,leftmargin=*,topsep=0em}
\setlist[enumerate]{noitemsep,leftmargin=*,topsep=0em}

